Forecasting mortality associated emergency department crowding

Emergency department (ED) crowding is a global public health issue that has been repeatedly associated with increased mortality. Predicting future service demand would enable preventative measures aiming to eliminate crowding along with it's detrimental effects. Recent findings in our ED indicate that occupancy ratios exceeding 90% are associated with increased 10-day mortality. In this paper, we aim to predict these crisis periods using retrospective data from a large Nordic ED with a LightGBM model. We provide predictions for the whole ED and individually for it's different operational sections. We demonstrate that afternoon crowding can be predicted at 11 a.m. with an AUC of 0.82 (95% CI 0.78-0.86) and at 8 a.m. with an AUC up to 0.79 (95% CI 0.75-0.83). Consequently we show that forecasting mortality-associated crowding using anonymous administrative data is feasible.

==> Makefile <==
.PHONY: all preddata

#################################################################################
# GLOBALS                                                                       #
#################################################################################

SHELL = /bin/zsh

plotdir = output/plots

TEXFILES = report/sections/abstract.tex\
	report/sections/conclusions.tex\
	report/sections/discussion.tex\
	report/sections/introduction.tex\
	report/sections/materials_and_methods.tex\
	report/sections/results.tex\
	report/sections/appendix.tex

TABLES = output/tables/metrics.tex\
	output/tables/duration.tex\
#	output/tables/data.tex

PLOTSPARAM = $(plotdir)/calmap-bed.png\
	$(plotdir)/calmap-sur.png\
	$(plotdir)/calmap-med.png\
	$(plotdir)/heatmap-bed.png\
	$(plotdir)/heatmap-med.png\
	$(plotdir)/heatmap-sur.png\
	$(plotdir)/aucorigin-bed.png\
	$(plotdir)/aucorigin-med.png\
	$(plotdir)/aucorigin-sur.png\
	
	
PLOTS2 = $(plotdir)/auc.png\
	$(plotdir)/balance.png\
	$(plotdir)/prcurve.png\
	$(plotdir)/shap.png\
	$(plotdir)/cohorts.png\
	$(plotdir)/f1.png\
	$(plotdir)/edor-example.png\
	$(plotdir)/bars.png\

PARAMNTB = notebooks/plot_calmap.ipynb\
	notebooks/plot_heatmap.ipynb\
	notebooks/plot_shap.ipynb\
	notebooks/plot_cohorts.ipynb

PLOTERRORMAP = $(plotdir)/errormap-med-lgbm-11-0-0.png\
	$(plotdir)/errormap-bed-lgbm-11-0-0.png\
	$(plotdir)/errormap-sur-lgbm-11-0-0.png\
	

probdir := data/processed/matrices/prob
pointdir := data/processed/matrices/point

POINTS = $(pointdir)/med-lgbm-8-0-0.csv\
	$(pointdir)/med-lgbm-9-0-0.csv\
	$(pointdir)/med-lgbm-10-0-0.csv\
	$(pointdir)/med-lgbm-11-0-0.csv\
	$(pointdir)/med-lgbm-12-0-0.csv\
	$(pointdir)/med-lgbm-13-0-0.csv\
	$(pointdir)/bed-lgbm-8-0-0.csv\
	$(pointdir)/bed-lgbm-9-0-0.csv\
	$(pointdir)/bed-lgbm-10-0-0.csv\
	$(pointdir)/bed-lgbm-11-0-0.csv\
	$(pointdir)/bed-lgbm-12-0-0.csv\
	$(pointdir)/bed-lgbm-13-0-0.csv\
	$(pointdir)/sur-lgbm-8-0-0.csv\
	$(pointdir)/sur-lgbm-9-0-0.csv\
	$(pointdir)/sur-lgbm-10-0-0.csv\
	$(pointdir)/sur-lgbm-11-0-0.csv\
	$(pointdir)/sur-lgbm-12-0-0.csv\
	$(pointdir)/sur-lgbm-13-0-0.csv\
	$(pointdir)/sur-guess-11-0-0.csv\
	$(pointdir)/bed-guess-11-0-0.csv\
	$(pointdir)/med-guess-11-0-0.csv\
	$(pointdir)/sur-guess-12-0-0.csv\
	$(pointdir)/bed-guess-12-0-0.csv\
	$(pointdir)/med-guess-12-0-0.csv\

	
PROBS = $(probdir)/med-lgbm-8-0-0.csv\
	$(probdir)/med-lgbm-9-0-0.csv\
	$(probdir)/med-lgbm-10-0-0.csv\
	$(probdir)/med-lgbm-11-0-0.csv\
	$(probdir)/med-lgbm-12-0-0.csv\
	$(probdir)/bed-lgbm-8-0-0.csv\
	$(probdir)/bed-lgbm-9-0-0.csv\
	$(probdir)/bed-lgbm-10-0-0.csv\
	$(probdir)/bed-lgbm-11-0-0.csv\
	$(probdir)/bed-lgbm-12-0-0.csv\
	$(probdir)/sur-lgbm-8-0-0.csv\
	$(probdir)/sur-lgbm-9-0-0.csv\
	$(probdir)/sur-lgbm-10-0-0.csv\
	$(probdir)/sur-lgbm-11-0-0.csv\
	$(probdir)/sur-lgbm-12-0-0.csv\
	$(probdir)/sur-guess-11-0-0.csv\
	$(probdir)/bed-guess-11-0-0.csv\
	$(probdir)/med-guess-11-0-0.csv\
	$(probdir)/sur-guess-12-0-0.csv\
	$(probdir)/bed-guess-12-0-0.csv\
	$(probdir)/med-guess-12-0-0.csv\
	
truedir := data/processed/true_matrices

TRUE = $(truedir)/bed.csv\
	$(truedir)/sur.csv\
	$(truedir)/med.csv\


MELTED = data/interim/melted.csv

MODEL = data/model/data-8.csv\
	data/model/data-9.csv\
	data/model/data-10.csv\
	data/model/data-11.csv\
	data/model/data-12.csv\
	data/model/data-13.csv\

INTERIM = data/interim/data.csv\

PREPROCESSED = data/preprocessed/targets.csv\
	data/preprocessed/calendar.csv\
	#data/preprocessed/beds.csv\
	#data/preprocessed/weather.csv\

PLOTS = $(PLOTERRORMAP) $(PLOTSPARAM) $(PLOTS2)

#################################################################################
# FUNCTIONS                                                                     #
#################################################################################

# $(call get_word, position_in_list, list) 
# Get nth element from {w1}-{w2}-{w3}-..-{wn}
define get_word
$(word $(1),$(subst -, ,$(basename $(notdir $(2)))))
endef

#################################################################################
# COMMANDS                                                                      #
#################################################################################

all: output/manuscript.pdf

preds: $(POINTS)

output/manuscript.pdf: $(PLOTS) $(TABLES) $(TEXFILES) report/manuscript.tex report/references.bib
	cd report\
	&& pdflatex manuscript\
	&& bibtex manuscript\
	&& pdflatex manuscript\
	&& pdflatex manuscript\
	&& cp manuscript.pdf ../output/manuscript.pdf\
	&& cp manuscript.pdf ~/Desktop/ed-bin-cat.pdf\
	&& open manuscript.pdf\
	

$(TABLES): output/tables/%.tex : notebooks/tab_%.ipynb $(TRUE) 
	cd notebooks\
	&& papermill $(notdir $<) /dev/null

$(PLOTS2): output/plots/%.png : notebooks/plot_%.ipynb $(TRUE) 
	cd notebooks\
	&& papermill $(notdir $<) /dev/null

$(PLOTERRORMAP): $(TRUE) notebooks/plot_errormap.ipynb 
	cd notebooks\
	&& papermill plot_$(call get_word,1,$@).ipynb /dev/null\
	 -p TARGET $(call get_word,2,$@)\
	 -p MODEL $(call get_word,3,$@)\
	 -p ORIGIN $(call get_word,4,$@)\
	 -p FS $(call get_word,5,$@)\
	 -p HPO $(call get_word,6,$@)

$(PLOTSPARAM): data/interim/data.csv $(PARAMNTB)
	cd notebooks\
	&& papermill plot_$(call get_word,1,$@).ipynb /dev/null -p TARGET $(call get_word,2,$@)

$(POINTS): notebooks/make_points.ipynb $(TRUE) $(PROBS)
	cd notebooks\
	&& papermill make_points.ipynb /dev/null

$(PROBS): scripts/test.py scripts/tutils.py $(MELTED)
	cd scripts\
	&& python test.py $(call get_word,1,$@) $(call get_word,2,$@) $(call get_word,3,$@) $(call get_word,4,$@) $(call get_word,5,$@) $(call get_word,6,$@);\

$(TRUE): notebooks/make_true_matrices.ipynb data/preprocessed/targets.csv
	cd notebooks\
	&& papermill make_true_matrices.ipynb /dev/null -p TARGET $(call get_word,1,$@)

$(MELTED): $(MODEL)
	cd notebooks\
	&& papermill make_melted.ipynb /dev/null

$(MODEL): $(INTERIM) notebooks/make_model_data.ipynb
	cd notebooks\
	&& papermill make_model_data.ipynb -p ORIGIN $(call get_word,2,$@) /dev/null

$(INTERIM): $(PREPROCESSED) notebooks/make_interim_data.ipynb
	cd notebooks\
	&& papermill make_interim_data.ipynb /dev/null

$(PREPROCESSED): data/preprocessed/%.csv : notebooks/make_%.ipynb
	cd notebooks\
	&& papermill $(notdir $<) /dev/null

data/raw/data.csv: notebooks/make_raw_data.ipynb
	cd notebooks\
	&& papermill make_raw_data.ipynb /dev/null

#################################################################################
# Helper Commands																#
#################################################################################

clean:
	rm -rf data/processed/*
	rm -r output/*

clear_report:
	rm report/manuscript.bbl
	rm report/manuscript.blg
	rm report/manuscript.log
	rm report/manuscript.out
	rm report/manuscript.aux

clear_notebooks:
	jupyter nbconvert notebooks/*.ipynb --clear-output --inplace

clear_results:
	rm -rf data/processed/matrices
	rm -rf data/processed/models
	rm -rf data/processed/studies
	rm -rf darts_logs
	rm logs/slurm/*
	rm logs/logger/*

==> output/tables/duration.tex <==
\begin{table}[H]
\caption{Distribution of crowding durations during days when even one day was crowded}
\begin{tabular}{lrrr}
\toprule
 & med & bed & sur \\
\midrule
count & 394.00 & 281.00 & 312.00 \\
mean & 4.72 & 4.60 & 3.84 \\
std & 2.70 & 2.44 & 2.32 \\
min & 1.00 & 1.00 & 1.00 \\
25\% & 2.00 & 3.00 & 2.00 \\
50\% & 4.50 & 4.00 & 3.50 \\
75\% & 7.00 & 6.00 & 5.00 \\
max & 13.00 & 12.00 & 11.00 \\
\bottomrule
\end{tabular}
\end{table}

